DASZL: Dynamic Action Signatures for Zero-shot Learning

There are many realistic applications of activity recognition where the set of potential activity descriptions is combinatorially large. This makes end-to-end supervised training of a recognition system impractical as no training set is practically able to encompass the entire label set. In this paper, we present an approach to fine-grained recognition that models activities as compositions of dynamic action signatures. This compositional approach allows us to reframe fine-grained recognition as zero-shot activity recognition, where a detector is composed "on the fly" from simple first-principles state machines supported by deep-learned components. We evaluate our method on the Olympic Sports and UCF101 datasets, where our model establishes a new state of the art under multiple experimental paradigms. We also extend this method to form a unique framework for zero-shot joint segmentation and classification of activities in video and demonstrate the first results in zero-shot decoding of complex action sequences on a widely-used surgical dataset. Lastly, we show that we can use off-the-shelf object detectors to recognize activities in completely de-novo settings with no additional training.

==> figures/bowling.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/temporal_v4.png}
  \caption{Attributes `open-one-arm', `throw-away' and `one-arm-swing' follow dynamic attribute pattern \texttt{(3):End} in a `bowling' sequences.}

\label{fig:temporal}
\end{figure}

==> figures/signature_statemachine.tex <==
\begin{figure*}[]
    \centering
    \begin{tikzpicture}[->,node distance=0.5cm,>=stealth']
        \node[state, initial] (end_1) {};
        \node[state, right=of end_1] (end_2) {};
        \node[state, accepting, right=of end_2] (end_3) {};
        
        \draw
            (end_1) edge [above] node{0} (end_2)
            (end_2) edge [loop above] node{0} (end_2)
            (end_2) edge [above] node{1} (end_3)
            (end_3) edge [loop above] node{1} (end_3)
            ;
    \end{tikzpicture}
    
    
    % \begin{tikzpicture}[->,node distance=0.5cm,>=stealth']
    %     \node[state, initial] (end_1) {a};
    %     \node[state, right=of end_1] (end_2) {b};
    %     \node[state, right=of end_2] (end_3) {c};
    %     \node[state, right=of end_3] (end_4) {d};
    %     \node[state, accepting, right=of end_4] (end_5) {e};
        
    %     \draw
    %         (end_1) edge [above] node{0} (end_2)
    %         (end_2) edge [above] node{0} (end_3)
    %         (end_3) edge [above] node{0} (end_4)
    %         (end_4) edge [above] node{1} (end_5)
    %         ;
    % \end{tikzpicture}
    
    % \vspace{0.4cm}
    
    \begin{tikzpicture}[->,node distance=1.75cm,>=stealth']
        \node[state, initial] (end_1) {0};
        % \node[state, right=of end_1] (end_2) {1};
        \node[state, draw=none, right=of end_1] (dots_1) {$\cdots$};
        \node[state, right=of dots_1] (end_t) {$t$};
        \node[state, draw=none, right=of end_t] (dots_2) {$\cdots$};
        \node[state, accepting, right=of dots_2] (end_T) {$T$};
        
        \draw
            (end_1) edge [bend left] node[above]{(1:1) / $p(1\mid x_1)$} (dots_1)
            (end_1) edge [bend right] node[below]{(1:0) / $p(0\mid x_1)$} (dots_1)
            % (end_2) edge [bend left] node[above]{2:1/$p(x_2, 1)$} (dots_1)
            % (end_2) edge [bend right] node[belop]{2:0/$p(x_2, 0)$} (dots_1)
            (dots_1) edge [bend left] node[above]{($t$:1) / $p(1 \mid x_t)$} (end_t)
            (dots_1) edge [bend right] node[below]{($t$:0) / $p(0 \mid x_t)$} (end_t)
            %(end_t) edge [bend left] node[above]{$(t+1)$:1/$p(1 \mid x_{t+1})$} (dots_2)
            %(end_t) edge [bend right] node[below]{$(t+1)$:0/$p(0 \mid x_{t+1})$} (dots_2)
            (end_t) edge [bend left] node[above]{$\cdots$} (dots_2)
            (end_t) edge [bend right] node[below]{$\cdots$} (dots_2)
            (dots_2) edge [bend left] node[above]{($T$:1) / $p(1 \mid x_T)$} (end_T)
            (dots_2) edge [bend right] node[below]{($T$:0) / $p(0 \mid x_T)$} (end_T)
            ;
    \end{tikzpicture}

    \caption{
        State machines implementing our dynamic attribute logic.
        Each edge is labeled with the token it accepts.
        TOP: The rule ``absent, then present" implemented as a machine that accepts one or more non-detections followed by one or more detections.
        % MIDDLE: The rule ``absent for first 75\%, then present for remaining 25\%",
        % instantiated for a length-4 sequence.
        BOTTOM: Transducer mapping a sequence to attribute detections.
        Edges are labeled with their input, their output, and their weight in that order.
    }
    
    \label{fig:signature-sm}
\end{figure*}
